Measurements of time-dependent CP asymmetries in B0 --> D(*)+D(*)- decays

We present new measurements of time-dependent CP asymmetries for B0 --> D(*)+D(*)- decays using (467 +/- 5) X 10^6 BB pairs collected with the BaBar detector located at the PEP-II B Factory at the Stanford Linear Accelerator Center. We determine the CP-odd fraction of the B0 --> D*+D*- decays to be R_perp = 0.158 +/- 0.028 +/- 0.006 and find CP asymmetry parameters for the CP-even component of the decay S_+ = -0.76 +/- 0.16 +/- 0.04 and C_+ = 0.00 +/- 0.12 +/- 0.02. We measure S = -0.63 +/- 0.36 +/- 0.05 and C = -0.07 +/- 0.23 +/- 0.03 for B0 --> D+D-, S = -0.62 +/- 0.21 +/- 0.03 and C = 0.08 +/- 0.17 +/- 0.04 for B0 --> D*+D-$, and S = -0.73 +/- 0.23 +/- 0.05 and C = 0.00 +/- 0.17 +/- 0.03 for B0 --> D+D*-. For the B0 --> D*+/-D-/+ decays, we also determine the CP-violating asymmetry A = 0.008 +/- 0.048 +/- 0.013. In each case, the first uncertainty is statistical and the second is systematic. The measured values for the asymmetries are all consistent with the Standard Model.

==> abstract.tex <==
We present new measurements of time-dependent $C\!P$ asymmetries for
$B^0 \rightarrow D^{(*)+}D^{(*)-}$ decays using $(467 \pm 5)\times 10^6$ $B{\kern 
0.18em\overline{\kern -0.18em B}{}}$ pairs collected with the \mbox{\slshape 
B\kern-0.1em{\smaller A}\kern-0.1em B\kern-0.1em{\smaller A\kern-0.2em R}} 
detector located at the PEP-II $B$ Factory at the Stanford Linear Accelerator 
Center.  We determine the $C\!P$-odd fraction of the $B^0 \rightarrow 
D^{*+}D^{*-}$ decays to be $R_\perp = 0.158 \pm 0.028 \pm 0.006$ and find $C\!P$ 
asymmetry parameters for the $C\!P$-even component of the decay $S_+ = -0.76 \pm 
0.16 \pm 0.04$ and $C_+ = 0.00 \pm 0.12 \pm 0.02$.  We measure $S = -0.63 \pm 0.36 
\pm 0.05$ and $C = -0.07 \pm 0.23 \pm 0.03$ for $B^0 \rightarrow D^+D^-$, $S = 
-0.62 \pm 0.21 \pm 0.03$ and $C = 0.08 \pm 0.17 \pm 0.04$ for $B^0 \rightarrow 
D^{*+}D^-$, and $S = -0.73 \pm 0.23 \pm 0.05$ and $C = 0.00 \pm 0.17 \pm 0.03$ for 
$B^0 \rightarrow D^+D^{*-}$.  For the $B^0 \rightarrow D^{*\pm}D^{\mp}$ decays, we 
also determine the $C\!P$-violating asymmetry $\mathcal{A} = 0.008 \pm 0.048 \pm 
0.013$.  In each case, the first uncertainty is statistical and the second is 
systematic.  The measured values for the asymmetries are all consistent with the 
Standard Model.

